The History of Digital Spam

Spam!: that's what Lorrie Faith Cranor and Brian LaMacchia exclaimed in the title of a popular call-to-action article that appeared twenty years ago on Communications of the ACM. And yet, despite the tremendous efforts of the research community over the last two decades to mitigate this problem, the sense of urgency remains unchanged, as emerging technologies have brought new dangerous forms of digital spam under the spotlight. Furthermore, when spam is carried out with the intent to deceive or influence at scale, it can alter the very fabric of society and our behavior. In this article, I will briefly review the history of digital spam: starting from its quintessential incarnation, spam emails, to modern-days forms of spam affecting the Web and social media, the survey will close by depicting future risks associated with spam and abuse of new technologies, including Artificial Intelligence (e.g., Digital Humans). After providing a taxonomy of spam, and its most popular applications emerged throughout the last two decades, I will review technological and regulatory approaches proposed in the literature, and suggest some possible solutions to tackle this ubiquitous digital epidemic moving forward.

==> ferrara-sb-bots.tex <==
\paragraph{How to create a social spam bot}
In the early days of online social media, over one decade ago, creating a bot was not a simple task: a skilled programmer would need to sift through various platforms' documentation to create a software capable of automatically interfacing with the platform and operate functions in a human-like manner. 
% 
These days, the landscape has completely changed: indeed, it has become increasingly simpler to deploy spam bots, so that, in some cases, no coding skills are required to setup accounts that perform simple automated activities: tech blogs often post tutorials and ready-to-go tools for this purposes. Various source codes for sophisticated social media bots can be found online as well, ready to be customized and optimized by the more technically-savvy users~\cite{kollanyi2016bots}. 
% 
We recently inspected same of the readily-available Twitter bot-making tools and compiled a non-comprehensive list of capabilities they provide \cite{bessi2016social}.
% 
Most of these bots can run within cloud services or infrastructures like Amazon Web Services (AWS) or Heroku, making it more difficult to block them when they violate the Terms of Service of the platform where they are deployed. 
% 
Finally, a very recent trend is that of providing Bot-As-A-Service (BaaS): Advanced conversational bots powered by sophisticated Artificial Intelligence are provided by companies like \textit{ChatBots.io} that can be used to carry digital spam campaigns and scale such operations by automatically engaging with online users. 

\paragraph{How to detect spam bots}
The detection of social spam bots in online social media platform has proven a challenging task. For this reason, it has attracted a lot of attention from the computing research community. Even DARPA, the U.S. \textit{Defense Advanced Research Projects Agency}, became interested and organized the 2016 DARPA Twitter Bot Detection~\cite{subrahmanian2016darpa}, with University of Maryland, University of Southern California, and Indiana University topping the challenge,  focused on detecting bots pushing anti vaccination campaigns.
% 
The literature on social spam bot detection has become very extensive. I tried to summarize the most relevant approaches in a survey paper recently appeared on the \textit{Communications of the ACM}~\cite{ferrara2016rise}: In that review, I proposed a simple taxonomy to divide the social spam bot detection approaches into three classes: \emph{(i)} bot detection systems based on social network information; \emph{(ii)} systems based on crowd-sourcing and leveraging human intelligence; \emph{(iii)} machine learning methods based on the identification of highly-predictive features that discriminate between bots and humans. I refer the interested reader to that review for a deeper analysis of this problem \cite{ferrara2016rise}.
